Linguistic Harbingers of Betrayal: A Case Study on an Online Strategy Game

Interpersonal relations are fickle, with close friendships often dissolving into enmity. In this work, we explore linguistic cues that presage such transitions by studying dyadic interactions in an online strategy game where players form alliances and break those alliances through betrayal. We characterize friendships that are unlikely to last and examine temporal patterns that foretell betrayal. We reveal that subtle signs of imminent betrayal are encoded in the conversational patterns of the dyad, even if the victim is not aware of the relationship's fate. In particular, we find that lasting friendships exhibit a form of balance that manifests itself through language. In contrast, sudden changes in the balance of certain conversational attributes---such as positive sentiment, politeness, or focus on future planning---signal impending betrayal.

==> style/preamble.tex <==
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
% \usepackage{bbm}
\usepackage{bm}
\usepackage{color}
%\usepackage[usenames,dvipsnames]{color}
\usepackage{comment}
\usepackage{tabularx}
\usepackage{environ}
\usepackage{textcomp}
\usepackage{float}
\usepackage{graphicx}
\usepackage{mathtools}
\usepackage{mdwlist}
\usepackage{microtype}
\usepackage{multirow}
% \usepackage[table]{xcolor}
\usepackage{multicol}
\usepackage{url}
\usepackage{latexsym}

% Do not put either of these (subfigure or subfloat) into the preamble
% - they clash.  Use them in the final LaTeX document
% Do not use times in the preamble!  It just causes problems.  If you
% want it, put it in your own document.
%\usepackage{times}

%\usepackage{ulem}

%comment out the following line, as it conflicts with aistats2012.sty
%\usepackage[font=small,labelfont=bf,tableposition=top]{caption}
\usepackage{nomencl}

\newcommand{\breakalign}{\right. \nonumber \\ & \left. \hspace{2cm}}

\newcommand{\topic}[1]{\underline{#1}}
\newcommand{\gem}[1]{\mbox{\textsc{gem}}}
\newcommand{\abr}[1]{\textsc{#1}}
\newcommand{\camelabr}[2]{{\scriptsize #1}{\textsc{#2}}}
\newcommand{\grammar}[1]{{\color{red} #1}}
\newcommand{\explain}[2]{\underbrace{#2}_{\mbox{\footnotesize{#1}}}}
\newcommand{\dir}[1]{\mbox{Dir}(#1)}
\newcommand{\bet}[1]{\mbox{Beta}(#1)}
\newcommand{\py}[1]{\mbox{\textsc{py}}(#1)}
\newcommand{\td}[2]{\mbox{\textsc{TreeDist}}_{#1} \left( #2 \right)}
\newcommand{\yield}[1]{\mbox{\textsc{Yield}} \left( #1 \right)}
\newcommand{\mult}[1]{\mbox{Mult}( #1)}
\newcommand{\wn}{\textsc{WordNet}}
\newcommand{\g}{\, | \,}
\newcommand{\G}[1]{\Gamma \left( \textstyle #1 \right)}
\newcommand{\LG}[1]{\log \Gamma \left( \textstyle #1 \right)}
\newcommand{\Pois}[1]{\mbox{Poisson}(#1)}
\newcommand{\pcfg}[3]{#1_{#2 \rightarrow #3}}
\newcommand{\grule}[2]{#1 \rightarrow #2}
\newcommand{\kl}[2]{D_{\mbox{\textsc{KL}}} \left( #1 \,||\, #2 \right)}

\newcommand{\digambig}[1]{\Psi \left( #1 \right) }
\newcommand{\digam}[1]{\Psi \left( \textstyle #1 \right) }
\newcommand{\ddigam}[1]{\Psi' \left( \textstyle #1 \right) }

\newcommand{\e}[2]{\mathbb{E}_{#1}\left[ #2 \right] }
\newcommand{\h}[2]{\mathbb{H}_{#1}\left[ #2 \right] }
\newcommand{\ind}[1]{\mathbb{I}\left[ #1 \right] }
\newcommand{\ex}[1]{\mbox{exp}\left\{ #1\right\} }
\newcommand{\D}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\elbo}{\mathcal{L}}

\newcommand{\hidetext}[1]{}
\newcommand{\ignore}[1]{}

\ifcomment
\newcommand{\nahocomment}[1]{  \colorbox{yellow}{   \parbox{.8\linewidth}{\scriptsize NAHO: #1}  }}
%\newcommand{\alvincomment}[1]{   \colorbox{violet}{\makebox[2em]{\strut\textcolor{yellow}{ACG}}} {   \colorbox{violet}{\textcolor{yellow}{\parbox{.8\linewidth}{\scriptsize Alvin: #1}  }}}}
\newcommand{\jbgcomment}[1]{  \colorbox{red}{   \parbox{.8\linewidth}{ JBG: #1}  }}
%\newcommand{\alvincomment}[1]{  \colorbox{violet}{  \parbox{.8\linewidth}{ ACG:  #1} }}


\newcommand{\yhcomment}[1]{  \colorbox{green}{  \parbox{.8\linewidth}{ YH:  #1}
  }}
\newcommand{\hhecomment}[1]{  \colorbox{blue}{  \parbox{.8\linewidth}{ HH:  #1}
  }}
\newcommand{\jjmcomment}[1]{  \colorbox{green}{  \parbox{.8\linewidth}{ John:  #1}
  }}
\newcommand{\tncomment}[1]{  \colorbox{blue}{  \parbox{.8\linewidth}{ TN:  #1}
  }}
\newcommand{\mnicomment}[1]{  \colorbox{green}{  \parbox{.8\linewidth}{ Mohit:  #1}  }}
\newcommand{\rscomment}[1]{  \colorbox{yellow}{  \parbox{.8\linewidth}{ Richard:  #1}  }}
\newcommand{\jszcomment}[1]{  \colorbox{green}{  \parbox{.8\linewidth}{ JSG:  #1}  }}
\newcommand{\ascomment}[1]{  \colorbox{blue}{  \parbox{.8\linewidth}{ AS:  #1}
  }}
\newcommand{\vecomment}[1]{  \colorbox{blue}{  \parbox{.8\linewidth}{ VE:  #1}  }}
\newcommand{\halcomment}[1]{  \colorbox{magenta!20}{  \parbox{.8\linewidth}{ Hal:  #1}  }}
\newcommand{\kgcomment}[1]{  \colorbox{blue}{  \parbox{.8\linewidth}{ Kim:  #1}  }}
\newcommand{\vancomment}[1]{  \colorbox{green}{  \parbox{.8\linewidth}{ VAN:  #1}  }}
\newcommand{\alvincomment}[1]{  \colorbox{violet}{  \parbox{.8\linewidth}{ VAN:  #1}  }}
\newcommand{\reviewercomment}[1]{  \colorbox{blue}{  \parbox{.8\linewidth}{Reviewer:  #1}  }}
\newcommand{\brscomment}[1]{  \colorbox{blue}{  \parbox{.8\linewidth}{BRS:  #1}  }}
\newcommand{\psrcomment}[1]{  \colorbox{yellow}{  \parbox{.8\linewidth}{PSR:  #1}  }}
\newcommand{\zkcomment}[1]{  \colorbox{cyan}{  \parbox{.8\linewidth}{ZK:  #1}  }}
\newcommand{\ctcomment}[1]{
  \colorbox{blue}{  \parbox{.8\linewidth}{CT:  #1}  }}
\newcommand{\swcomment}[1]{ \colorbox{yellow}{ \parbox{.8\linewidth}{ SW: #1}
  }}
\newcommand{\shaycomment}[1]{  \colorbox{yellow}{  \parbox{.8\linewidth}{SBC:  #1}  }}
\else
\newcommand{\nahocomment}[1]{ }
\newcommand{\alvincomment}[1]{ }
\newcommand{\jbgcomment}[1]{ }
\newcommand{\yhcomment}[1]{ }
\newcommand{\jjmcomment}[1]{ }
\newcommand{\hhecomment}[1]{ }
\newcommand{\tncomment}[1]{ }
\newcommand{\mnicomment}[1]{ }
\newcommand{\ascomment}[1]{ }
\newcommand{\vecomment}[1]{ }
\newcommand{\halcomment}[1]{ }
\newcommand{\kgcomment}[1]{ }
\newcommand{\brscomment}[1]{ }
\newcommand{\reviewercomment}[1]{ }
\newcommand{\zkcomment}[1]{ }
\newcommand{\jszcomment}[1]{ }
\newcommand{\ctcomment}[1]{ }
\newcommand{\swcomment}[1]{ }
\newcommand{\psrcomment}[1]{ }
\newcommand{\vancomment}[1]{ }
\newcommand{\shaycomment}[1]{ }
\fi

\newcommand{\email}[1]{\begin{small} \url{#1} \end{small}}
\newcommand{\smallurl}[1]{ \begin{scriptsize}\url{#1}\end{scriptsize}}
\newenvironment{compactenum}{ \begin{enumerate*} \small }{ \end{enumerate*} }

\NewEnviron{smalign}{
\vspace{-.6cm}
\begin{small}
\begin{align}
  \BODY
\end{align}
\end{small}
\vspace{-.6cm}
}

\definecolor{grey}{rgb}{0.95,0.95,0.95}

